Accurate and Robust Localization Techniques for Wireless Sensor Networks

The report focuses on three areas in particular: the first is the Received Signal Strength indicator technique, Direction of Arrival technique, and the integration of two algorithms, RSS and DOA, in order to build a hybrid, more robust algorithms. In the Received Signal Strength (RSS), the unknown node location is estimated using trilateration. This report examines the performance of different estimators such as Least Square, Weighted Least Square, and Huber robustness in order to obtain the most robust performance. In the direction of arrival (DOA) method, the estimation is carried out using Multiple Signal Classification (MUSIC), Root-MUSIC, and Estimation of Signal Parameters Via Rotational Invariance Technique (ESPRIT) algorithms. We investigate multiple signal scenarios utilizing various antenna geometries, which includes uniform linear array (ULA) and uniform circular array (UCA). Specific attention is given for multipath scenarios in which signals become spatially correlated (or coherent). This required the use of pre-processing techniques, which include phase mode excitation (PME), spatial smoothing (SS), and Toeplitz. Further improvements of existing localization techniques are demonstrated through the use of a hybrid approach in which various combinations of RSS and DOA are explored, simulated, and analyzed. This has led to two major contributions: the first contribution is a combined RSS/DOA method, based on UCA, which has the tolerance of detecting both uncorrelated and coherent signals simultaneously. The second major contribution is a combined Root-MUSIC/Toepltiz method, based on UCA, which is outperforms other techniques in terms of increased number of detected signals and reduced computationally load.

==> Declare.tex <==
\chapter{Declaration and Copyright}
{
\section*{Declaration}
I declare that the work in this report was carried out in accordance with the regulations of Khalifa University of Science, Technology, and Research. The work is entirely my own except where indicated by special reference in the text. Any views expressed in the report are those of the author and in no way represent those of Khalifa University of Science, Technology, and Research. No part of the report has been presented to any other university for any degree.
\vspace*{1cm}

\noindent SIGNED: \dotfill \hspace{0.2cm}DATE: \dotfill
}
\vfill
\begin{singlespace}
{\section*{Copyright \copyright} 
No part of this report may be reproduced, stored in a retrieval system, or transmitted, in any
form or by any means, electronic, mechanical, photocopying, recording, scanning or otherwise, without prior written permission of the author. The thesis may be made available for consultation in Khalifa University of Science, Technology, and Research Library and for inter-library lending for use in another library and may be copied in full or in part for any bona fide library or research worker, on the understanding that users are made aware of their obligations under copyright, i.e. that no quotation and no information derived from it may be published without the author's prior consent.
}
\end{singlespace}




==> ch4/Sheet1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{crccrr}
    \toprule
    \textbf{N} & \textbf{} & \textbf{Magnitude of the Roots} & \textbf{Radial distance from the unit circle} & \textbf{} & \textbf{} \\
    \midrule
    \multirow{2}[2]{*}{\textbf{4}} & \multicolumn{1}{c}{-10o} & 0.98  & 0.2   & \multicolumn{1}{c}{-10.53o} & \multicolumn{1}{c}{0.53o} \\
          & \multicolumn{1}{c}{10o} & 0.97  & 0.3   & \multicolumn{1}{c}{9.67o} & \multicolumn{1}{c}{0.33o} \\
    \multirow{2}[2]{*}{\textbf{8}} & \multicolumn{1}{c}{-10o} & 1     & 0     & \multicolumn{1}{c}{9.97o} & \multicolumn{1}{c}{10.01o} \\
          & \multicolumn{1}{c}{10o} & 1     & 0     & \multicolumn{1}{c}{-9.93o} & \multicolumn{1}{c}{-9.99 o} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> ch6/chapter6.tex <==
%%\begin{document}
\chapter{Graphical User Interface}
\label{Graphical User Interface}
Graphical user interfaces GUIs is a graphical display that allows the users to easily interact with a software through the use of different icons and indicators known as components. It gives “point-and-click” control for different applications which allows the users to have many options to choose and control the follow of the program.  MATLAB provides GUI that can deliver any task or provide different calculations, data, graphs and plots.  There are varieties of components such as toolbars, push buttons, menus, list boxes, sliders, and radio buttons \cite{moore_matlab_2014}.
 
For this project, three GUIs were designed to allow the user to explore the localization techniques. Actually, there is main GUIs from which the user chooses one of the three techniques and then a new window is opened that corresponds to the chosen technique.  

\section{Main GUIs window}
The main window page contains three push buttons that are named RSS, DOA and Hybrid as shown in Figure 1.

\begin{figure} [h]
       \centering
        \includegraphics[width=1\textwidth,clip]{ch4/figures/gui1.eps}
        \caption[GUI main window]{GUI main window}
		 \label{Fig:gui1}
\end{figure} 

\section{RSS technique GUIs}
In this GUIs, the user enters a location of the node which is two numbers which corresponds to the $x$ and $y$ coordinates and these numbers are between the (1-30 m). The user should enter 4 positions for the nodes. Then, the user has two choices to choice the desired estimators, either LS or WLS. After that, the estimated and the actual points are displayed on the window. Also, two graphs will be in the GUIs the first one shows the location of the node in the environment along with the actual and the estimated positions. Another graph shows the plot of the RMSE versus SNR.  The user can clear the inputs and the graph to restart a new simulation.   Finally, the user can move to the next GUIs or go back to the main window.   Figure \ref{Fig:gui2}, shows the WLS estimator results and node locations. The estimated point is in red and the actual location is in green. The RMSE versus SNR graph is shown and the $x$,$y$ coordinates are obtained and displayed below in the graph.

\begin{figure} [h]
       \centering
        \includegraphics[width=1\textwidth,clip]{ch4/figures/gui2.eps}
        \caption[RSS GUI results]{RSS GUI results}
		 \label{Fig:gui2}
\end{figure} 

\section{DOA technique GUIs}
If the user chooses the “next” pushbutton in the RSS technique GUIs, the user enters the number of the incoming signals, angles of the arrival and the number of elements and snapshots. Then, the user chooses the environment if correlated or uncorrelated along with array geometry if it is ULA or UCA. In the case of the correlated environment, the user can choose from the two types of spatial smoothing which are FBSS and FSS. After that, the angular spectrum is shown in the window.  The user can clear everything and start a new simulation.  Finally, the user can move to the next GUIs which is the hybrid or go back to the previous GUIs window. Figure \ref{Fig:gui3}, shows the GUIs for the DOA and sample of the results which is taken in the correlated UCA with FSS.

\begin{figure} [h]
       \centering
        \includegraphics[width=1\textwidth,clip]{ch4/figures/gui3.eps}
        \caption[DOA GUI results]{DOA GUI results}
		 \label{Fig:gui3}
\end{figure} 

\section{Hybrid technique GUIs}
The last GUIs is the hybrid technique. The user types the location of the node (i.e. $x$ and $y$ coordinates) which lay in the range (1-30 m). Then, the user has five choices to choice the Hybrid techniques. The techniques are Hybrid with one hybrid node, Hybrid LS and WLS, Hybrid two lines and for the correlated environment the Hybrid with spatial smoothing. After that, by choosing one technique at the time, the RMSE versus SNR graph is displayed in the window. Another graph is shown for the positions of the nodes. The actual number for the positions is printed on the GUIs window. Three pushbuttons are in the window, one to go back to the previous GUIs and the one return to main. The last one allows the user to reset to the default values, and starts new test. Figure \ref{Fig:gui4}, shows the results using Hybrid LS and the node positions.

\begin{figure} [h]
       \centering
        \includegraphics[width=1\textwidth,clip]{ch4/figures/gui4.eps}
        \caption[Hybrid GUI results]{Hybrid GUI results}
		 \label{Fig:gui4}
\end{figure} 
